EdgeToll: A Blockchain-based Toll Collection System for Public Sharing of Heterogeneous Edges

Edge computing is a novel paradigm designed toimprove the quality of service for latency sensitive cloud applications. However, the state-of-the-art edge services are designedfor specific applications, which are isolated from each other.To better improve the utilization level of edge nodes, publicresource sharing among edges from distinct service providersshould be encouraged economically. In this work, we employ thepayment channel techniques to design and implement EdgeToll,a blockchain-based toll collection system for heterogeneous public edge sharing. Test-bed has been developed to validate theproposal and preliminary experiments have been conducted todemonstrate the time and cost efficiency of the system.

==> backups.tex <==
each user, proxy and edge will be provided an address in Ethereum. Given the address in Ethereum, like the account in bank, the transaction can be established. Payment channel is a great technique to improve the efficiency of transaction. In the proposed toll collections system, there are mainly two kinds of payment channel: one is between user and proxy which is for user pay for the proxy, and one is between proxy and edge, which is for proxy pay for the edge. Essentially. There are no difference in two kinds of payment channel but recipients are different.
    
Usually, edge should send register request to proxy and the payment channel between edge and proxy will be established (Proxy will evaluate the condition of edge and deposit certain amount of token, in the experiment, the amount is set 1 ether fixed). And if user want to use the computational service, user should open a payment channel for proxy and deposit token in it. The amount can be random but 1 ether fixed in this experiment. Assumed that users have several tasks to accomplish, for example, a simple face detection task, which mobile terminal (users) can not finish but edges can. The task will detect humans' face In the experiment group based on toll collection system, the user will open a payment channel for proxy first so that the request to proxy will not be blocked (the payment channel in proxy and edge has existed). Then user will search for available edges report the list to proxy. Proxy will analyze the condition of edge and return an optimal edge to user. Then user connect to the access point launched by the selected edge. After edge finish the computing, the result will be send to user through network. After user confirm the result, user will use its private key to sign and send a signature splitting the token in smart contract to Proxy. Proxy will check the legality of signature and send a equal amount signature to edge. At some time, proxy and edge will withdraw the money from smart contract using the signature. But for the experimental group without toll collection system, the user build payment channel and send signature directly to connected edge. Because the uncertainty of mobile terminal, the user may move to the next location and the connection between user and edge may terminated. Considering the problems above, user should need to send ether directly to the edge's account in Ethereum. Or they build a payment channel, once a transaction is done, edge will withdraw token from the payment channel. In our experiment, we assume they build payment channel. And the experiments will change tasks user have and measure the time cost (s) and gas fee (a measurement of cost in transaction of Ethereum). By comparing the data with the increasing of user's tasks, the advantage of toll collection system can be shown.

\item Edge Revenue Maximization: this experiment considers the scenarios when multiple users are competing for limited edge resources.  
    Edges usually care about the revenue because of the rentability. When the market is in equilibrium, the revenue of edges may be determined by the market. But when the balance was broken by unbalanced supply and demand relationship, the revenue may be different. So in our experiment, we aim to measure the profit condition of edges when the edges are limited and many users have to connect to one edge. So in this condition, proxy in EdgeToll collection system may collect all users condition and help edge to decide which user to connect first. The result may be determined by many factors and in this experiment we only focus on the price user offered. By determining the priority of applied users, the proxy can maximize the edges' revenue. If without the proposed system, the edge may be hard to analyze and determined the order of users. Edge may just select user by the applying time. Therefore, the proxy can optimize the revenue results in some extends.
    
    If without the proposed system, the edge may be hard to analyze and determined the order of users. Edge may just select user by the applying time. Therefore, the proxy can optimize the revenue results in some extends.
    
    
    Besides the time cost, gas fee and the revenue of edges in congestion case, another metrics will be measured -- saved price. The index comes from that user will propose a fixed expected price for that face detection task, and after proxy analyze the condition of edge, it will finally return a selected edge and price for that user. That provided price is usually smaller than the proposed price, so the difference is the saved price. The saved price can make positive contribution to users and edges. The larger the index is , the more the toll collection system can contribute to user. The proxy can help user to choose a suitable edge when there are many various and heterogeneous edges, compared to user choose a edge randomly, the decision can be smarter. The saved price measures how much price benefit can proxy contribute to user. 
    
    
    The saved price can make positive contribution to users and edges. The larger the index is , the more the toll collection system can contribute to user. The proxy can help user to choose a suitable edge when there are many various and heterogeneous edges, compared to user choose a edge randomly, the decision can be smarter. The saved price measures how much price benefit can proxy contribute to user. 
    
    

the diagram of Total time cost versus different amount of tasks. Fig. \ref{fig:totaltime} measures how the total time cost with two different ways. Use an example to illustrate the mechanism of proposed EdgeToll collection system. For example, a mobile user A want to finish 50 complex and difficult computational tasks. First, user need to build payment channel to proxy and we assume that all available edges have registered. Considering the mobility of A and the optimization of tasks, so at the beginning of each task, user A need to search for available edges (each edge is an access point), and send the available edges list to proxy to wait for the selected edge. Once edge is selected, send task to it and receive results. Once the task is done, send a signature splitting the coin stored in contract. So the working flow above will repeat for 50 times. One thing to mention is in the working process of proposed EdgeToll collection system, there are no on-blockchain operation until the final task. In the final task, proxy and edges use signature to split the cryptocurrency. Once the signature is used to split coin, the channel will be cancelled. If user want to finish 50 tasks again, user need to build payment channel to proxy first and edges should register again. But for the transaction way without toll collection system, once A get a result from edge, A need to sign a transaction to edge B which need to be broadcasted into P2P network and written in block. The total time cost measures at different workload (different amount of tasks of user), how much time will need to solve the tasks of user. The total time cost increase linearly as the increasing of numbers of users' task. When the amount of users' task is small, e.g. 1 task, the total time cost of proposed system may be expensive than the time cost of traditional way. However, as the increase of amount of tasks, the time cost of proposed system begin to show the advantage. When the amount of users' task is 50 and block time equals 15s (Rinkeby), the difference of time cost is 1185s, more than two times of the time cost in proposed EdgeToll system. When the block time of blockchain network increase, the difference of time cost will also increase. When blocktime is set 5s, 10s and 15s, the highest difference is 306s, 552s, 1185s repectively and 24\%, 56\%, 110\% from the proposed system time cost respectively.


is the diagram of gas fee in transaction versus different amount of tasks. Fig. \ref{fig:gasfee} illustrates the transaction cost in Ethereum. Like BitCoin, every online transaction written in the block need some fee to pay for the miner. gas is not the fee, but use gas can estimate fee using gas price. So gas is a estimation of transaction cost. Like the example above, the experiment have two groups to measure. At different workload of user (different amount of tasks), measure how the gas cost change. The result is in line with expectations. The gas cost of toll collection system remain constant but the other gas cost increase as the increment in users' tasks. This is because no matter how many tasks user have, if user use toll collection system, only 4 transaction need to be broadcasted. Two for user and proxy respectively deposit money in smart contract and two for proxy and edge to withdraw money from smart contract. But for traditional way, user A first deposit cryptocurrency into smart contract. Then it connected to selected edge B and transmit the computational task. Once a task is done, A need to search for new edge to compute for next task because of the mobility of user. So A sign a signature to edge and edge withdraw the currency. A can not directly send currency B because B may do not compute for A or A do not pay for B. It's a trust problem and will not be talked about carefully. From the graph, the system is powerful because this shows that the transaction cost will not increase with the workload of computational tasks. The gas fee of proposed toll collection system usually remain constant, so different gas price only influence the amount of fee but not change the increasing tendency. But if the transaction system use traditional way (user directly send money to edge for transaction), the total gas fee may increase as the total number of tasks increase. And as the gas price increase, the increasing slope will also become larger. When user have a heavy workload e.g. 50 tasks and high gas price ( gas price = 7 Gwei), the total gas fee of traditional way is nearly 40 times larger than the fee of toll collection system. Even in the low gas price ( gas price = 1 Gwei), when workload of user is large (50 tasks), the gas fee can also be 6 times larger than the total gas fee of toll collection system. Therefore, the toll collection system can significantly reduce the gas fee of transaction. Only when the workload of user is small, e.g. only 1 task, The gas fee of toll collection system may be slightly greater than the gas fee without system. 


Fig. \ref{fig:costsaving} is the diagram of .Fig. \ref{fig:costsaving} shows the overall cost savings when the proposed EdgeToll system has been implemented. The working flow of toll collection system is below: mobile terminal user search for available edges and report the available list to proxy. proxy will compare the price of the edge and return a optimal price. For each task at different time, the price will change based on the usage condition of edges. The price of edge may vacillate among a range because of the workload and memory usage. For the toll collection system, proxy can access the price of different edges and return an optimal edge to connect. But if without system, user may randomly select an edge to connect and maybe that edge is not the optimal choice. Every time user will propose a fix price for each task and use fix price subtract edges' optimal price, the result will be the saved price. The experiment measures the saved price for different number of tasks. The diagram shows that the toll collection system can significantly reduce users' cost for tasks. Because the price history of cloud may vacillate in a range, so we grab some data in amazon web service, and use some random function to simulate it. 
